AgenticRec: A Recommendation-Oriented Agentic Framework with Progressive Tool-Integrated Reasoning Optimization

Recommender agents built on Large Language Models offer a promising paradigm for personalized recommendation. However, existing agents typically suffer from a misalignment between their tool-integrated reasoning trajectories and recommendation feedback, limiting their ability to distinguish fine-grained user preferences. To address these challenges, we propose AgenticRec, an agentic recommendation framework that formulates recommendation as a tool-integrated reasoning process over a recommendation-oriented tool suite. Built upon this framework, we further develop a dedicated two-stage training paradigm tailored for recommender agents. In the first stage, we introduce Recommendation-Oriented Trajectory Activation, optimize the agentic recommendation ability under implicit feedback. In the second stage, Progressive Preference Refinement further refines the agent through bidirectional preference reasoning over self-bootstrapped hard pairs, progressively sharpening preference boundaries. Theoretical analysis and extensive experiments demonstrate the effectiveness of AgenticRec. Our code is available at https://anonymous.4open.science/r/AgenticRec-FB16.

==> Sections/Problem_Definition.tex <==
\section{Problem Formulation}
\label{sec:problem_definition}
Following prior recommender agent setting~\cite{RecMind,iAgent}, given a user interaction history $x_u=[v_1,v_2,\dots,v_t]$ and a candidate set $\mathcal{C}=\{c_1,c_2,\dots,c_n\}$, the recommender agent aims to generate a ranked list
$r_K=[c_{\sigma(1)},c_{\sigma(2)},\dots,c_{\sigma(K)}]$
of the Top-$K$ items that are most likely to match the user’s preferences, where $\sigma(\cdot)$ denotes the ranking order over candidate items and $K \le n$.

Our goal is to learn an agent policy $\pi_\theta$ that maximizes the expected list-wise utility under real-world feedback $y$:
\[
\max_{\theta}\ \mathbb{E}_{(x_u,\mathcal{C},y)\sim\mathcal{D}}\big[R(r_K, y)\big], 
\]
where $R(\cdot)$ measures the ranking quality induced by implicit feedback (e.g., NDCG@K).
